Citizen Scientist Community Engagement with the HiggsHunters project at the Large Hadron Collider

The engagement of Citizen Scientists with the HiggsHunters.org citizen science project is investigated through analysis of behaviour, discussion, and survey data. More than 37,000 Citizen Scientists from 179 countries participated, classifying 1,500,000 features of interest on about 39,000 distinct images. While most Citizen Scientists classified only a handful of images, some classified hundreds or even thousands. Analysis of frequently-used terms on the dedicated discussion forum demonstrated that a high level of scientific engagement was not uncommon. Evidence was found for a emergent and distinct technical vocabulary developing within the Citizen Science community. A survey indicates a high level of engagement and an appetite for further LHC-related citizen science projects.

==> frequencies.tex <==
slice && 1570\\
view && 1458\\
ocv && 1238\\
lines && 1131\\
muon && 1031\\
possible && 958\\
energy && 876\\
tracks && 850\\
particles && 848\\
center && 842\\
line && 836\\
normal && 719\\
vertex && 717\\
white && 707\\
muons && 613\\
red && 607\\
green && 597\\
mark && 595\\
off-center && 551\\
o\'clock && 548\\
more && 539\\
track && 528\\
detector && 500\\
blue && 425\\
yellow && 422\\
quark && 408\\
particle && 368\\
computer && 358\\
vertices && 351\\
image && 351\\

#ocv && 6305\\
#weird && 1341\\
#missingmuon && 887\\
#photon && 834\\
#muon && 732\\
#bottom && 642\\
#multiple && 545\\
#bundle && 527\\
#lots && 471\\
#messy && 449\\
#energy && 447\\
#diametric && 402\\
#mess && 302\\
#bottomquark && 292\\
#toughie && 278\\
#electron && 209\\
#wideangle && 187\\
#interesting && 164\\
#muons && 153\\
#jet && 145\\
#yellowfencepanels && 107\\
#sim && 103\\
#punch-through && 98\\
#red && 93\\
#bottomquarkandphoton && 87\\
#missing && 86\\
#higgszcandidates && 83\\
#energydeposit && 78\\
#blue && 73\\
#simulation && 72\\


==> simul.tex <==

\section{Simulation and image reconstructon details}
\label{sec:simul}

%% AMI: e2906, 17.2.13.4, MC12JobOpts-00-12-91_v9, Pythia 8.175 + Photospp, 
%% TWiki (https://twiki.cern.ch/twiki/bin/viewauth/AtlasProtected/AtlasMcProductionMC12#Production_validation_releases): MG5 1.5.2
Calibration $Z (\to \mu^+ \mu^-) + H (\to \phi \phi)$ events were generated using \texttt{MadGraph}-5.1.5.2~\cite{MadGraph5} 
interfaced to \texttt{Pythia}-8.175 \cite{pythia6,pythia8} 
using the \texttt{AU2} tune~\cite{Pythia8tunes} of \texttt{Pythia} parameters with the \texttt{CTEQ6L1}~\cite{CTEQ6} 
PDF set. The $\phi$ is a pseudoscalar boson, i.e. a spinless particle with negative parity.

%%  MG5_aMC@NLO v2.2.2 [10] at Leading Order interfaced to the Pythia 8.186 [5] parton shower model. The A14 tune is used together with the NNPDF2.3LO PDF set [14]. The EvtGen v1.2.0 program [3] is used for properties of the bottom and charm hadron decays. The W/Z + jets events are normalized to the NNLO cross sections ((see [[https://twiki.cern.ch/twiki/bin/view/AtlasProtected/CrossSectionHighOrder for reference).''

%% Photos++ version 3.52 [11] is used for QED emissions from electroweak vertices and charged leptons


They were passed through ATLAS simulation infrastructure~\cite{SOFT-2010-01}, 
and simulated pileup events from the same and surrounding bunch crossings were added, 
along with modelled detector noise, corresponding to the same luminosity profile as the 2012 data sample.

Tracks and vertices were reconstructed as described in Ref.~\cite{Aad:2015rba}.
In particular, the tracking was extended from 
the ATLAS default impact parameter of 1\,cm, to\,10 cm. 
The total simulation and reconstruction time was about 10\,minutes per event, 
or $\sim$1 CPU-year. (This was spread out to many computers on the ATLAS grid
to process $\sim$50k events in $\sim$2 days.) 

The total data size of $\sim$250\,GB was then reduced to $\sim$100 GB of images. 
These images were made using the ATLAS Atlantis event display~\cite{atlantis,Taylor:2005wi}.
Selections were applied to reduce the amount of visual information (clutter) 
shown in each image, while still allowing vertices to be seen. 
Only tracks with $\pt>2$~\GeV and starting $> 0.5$~mm in the transverse plane from
the beamline were shown (since there are $\sim$1000's of low \pt, tracks originating from the interaction point.) 
Tracks that start more than 20\,cm from the center 
of the detector or the selected collision point in the direction along 
the beamline are not drawn. 
To reduce the number of fake tracks, they must have at least seven 
hits in the silicon strip tracker. Vertices shown must have at least three 
tracks. Muon tracks must have $\pt > 10$~\GeV, and 
jets of hadrons must have $\pt > 40$~\GeV. 
Other objects (photons, electrons, bottom quark jets, etc.) are drawn as
long as they have $\pt > 5$~\GeV.

The images were displayed using a non-linear 
radially dependent fish-eye transform of the form
\[
r^\prime = \frac{a r}{m(1 + c r)}
\]
where $a$, $c$ and $m$ are real positive constants,
and $r$ is the radius in pixels in the $x-y$ view.
This transform serves to increase viewers' attention to and precision within
the central tracking layers of the ATLAS detector.

